AI Risk Management Should Incorporate Both Safety and Security

The exposure of security vulnerabilities in safety-aligned language models, e.g., susceptibility to adversarial attacks, has shed light on the intricate interplay between AI safety and AI security. Although the two disciplines now come together under the overarching goal of AI risk management, they have historically evolved separately, giving rise to differing perspectives. Therefore, in this paper, we advocate that stakeholders in AI risk management should be aware of the nuances, synergies, and interplay between safety and security, and unambiguously take into account the perspectives of both disciplines in order to devise mostly effective and holistic risk mitigation approaches. Unfortunately, this vision is often obfuscated, as the definitions of the basic concepts of "safety" and "security" themselves are often inconsistent and lack consensus across communities. With AI risk management being increasingly cross-disciplinary, this issue is particularly salient. In light of this conceptual challenge, we introduce a unified reference framework to clarify the differences and interplay between AI safety and AI security, aiming to facilitate a shared understanding and effective collaboration across communities.

==> sections/privacy_fairness.tex <==
\section{Other Relevant Disciplines}
\label{sec:other_disciplines}


The examination in this paper may be extended more broadly to many other important disciplines, which can be strongly related to AI risk management but not necessarily under the umbrella of either AI safety or AI security. For each of those disciplines, there could be unique challenges studied by its own dedicated communities with different methodologies and mindsets. Stakeholders need to strive to build a holistic and inclusive risk management framework that can effectively coordinate efforts from all these disciplines to work toward the shared goal of making the adoption of AI beneficial for humanity at large. This section briefly discusses fairness and privacy while also acknowledging other related disciplines not covered in this section.


%As an example, this section briefly walks through studies of fairness and privacy, discussing their relevance and differences to safety and security. We also acknowledge the existence of other such disciplines not covered in this section. %Just as it is important to ensure consistent investment in security and safety, it is equally important to invest in other specific areas of risk.

\textbf{Fairness} generally concerns the equitable and just distribution of both the benefits and risks of AI technologies. In practice, standards and definitions of fairness can greatly vary across different applications~\citep{barocas2023fairness}. The definitions of fairness can also be subjective~\citep{grgic2018human}, culturally influenced~\citep{greenberg2001studying}, and even conflicting~\citep{kleinberg2016inherent}. The intersections of AI fairness with safety and security considerations are noteworthy. For example, deploying LLMs without proper consideration of fairness could perpetuate existing biases and stereotypes prevalent on the internet and in society~\citep{welbl2021challenges}, a concern more aligned with safety considerations. Regarding security, adversaries can easily manipulate the system's behavior to introduce bias~\citep{solans2020poisoning, chang2020adversarial, mehrabi2021exacerbating}.  Nonetheless, we also discuss in \Cref{app:remark_on_fairness} that fairness issues can often be complicated and extend beyond the realms of safety and security. 


%\yang{@Weijie, could you please help proofread and expand (if needed) the paragraph on privacy? Please feel free to push more details to \Cref{app:remark_on_privacy} if needed. Thanks!}

\textbf{Privacy} also presents a rather complex challenge in AI risk management. It is a comprehensive concept that plays a crucial role in protecting fundamental values like human autonomy and dignity. Although the definition of privacy~\citep{solove2010understanding} and strategies for its protection vary across cultural contexts, individual preferences, and application scenarios, several common privacy-enhancing techniques are widely recognized. These include, but are not limited to, anonymization~\citep{bayardo2005data}, removing personally identifiable information~\citep{pii}, differential privacy~\citep{dwork2014algorithmic}, and secure multi-party computation~\citep{yao1986generate, goldreich1998secure}. Privacy-related risks encompass a broad spectrum that intersects with safety and security concerns to varying degrees. Certain privacy breaches directly expose safety or security risks, like chatbots accidentally disclosing user data~\citep{chatgpt_leak_1, chatgpt_leak_2} and intentional data extraction attacks by adversaries~\citep{carlini2021extracting, carlini2023extracting, nasr2023scalable}.
On the other hand, some privacy risks such as membership inference~\citep{shokri2016membership} and the auditing of certain privacy mechanisms~\citep{jagielski2020auditing, steinke2023privacy} primarily pertain to traditional privacy concerns, but they can also indirectly cause safety and security vulnerabilities~\citep{yao2023survey}. A thorough
exploration of privacy requires a more nuanced discussion, which falls beyond the scope of this paper. For an in-depth understanding of privacy definitions and risks, we recommend referring to the NIST Privacy Framework~\citep{nistframework} and a recent survey by~\citet{Cummings2024Advancing}.







